Automatic Image-Level Morphological Trait Annotation for Organismal Images

Morphological traits are physical characteristics of biological organisms that provide vital clues on how organisms interact with their environment. Yet extracting these traits remains a slow, expert-driven process, limiting their use in large-scale ecological studies. A major bottleneck is the absence of high-quality datasets linking biological images to trait-level annotations. In this work, we demonstrate that sparse autoencoders trained on foundation-model features yield monosemantic, spatially grounded neurons that consistently activate on meaningful morphological parts. Leveraging this property, we introduce a trait annotation pipeline that localizes salient regions and uses vision-language prompting to generate interpretable trait descriptions. Using this approach, we construct Bioscan-Traits, a dataset of 80K trait annotations spanning 19K insect images from BIOSCAN-5M. Human evaluation confirms the biological plausibility of the generated morphological descriptions. We assess design sensitivity through a comprehensive ablation study, systematically varying key design choices and measuring their impact on the quality of the resulting trait descriptions. By annotating traits with a modular pipeline rather than prohibitively expensive manual efforts, we offer a scalable way to inject biologically meaningful supervision into foundation models, enable large-scale morphological analyses, and bridge the gap between ecological relevance and machine-learning practicality.

==> figures/sae_case_study_ex.tex <==
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/insect_imgs/sae_case_study_ex1.pdf}
        \caption{Neuron 4852 in SAE gets activated at wings of insects (bottom), original image on top. The labels denote the highest annotated taxonomic level.}
        \label{fig:sae_case_study_ex1}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/insect_imgs/sae_case_study_ex2.png}
        \caption{Neuron 13860 gets activated at the antenna of insects. The labels denote the highest annotated taxonomic level.}
        \label{fig:sae_case_study_ex2}
    \end{subfigure}
    \caption{Visualization of neuron activations.}
\end{figure}

==> tables/dataset_ablation_trait_thresh.tex <==
\begin{table}[htbp]
\centering
\caption{Statistics of latents obtained at different thresholds for species classification rationale generation (1000 input images). \vardaan{update stats for 100 images}}
\begin{tabular}{@{}lll@{}}
\toprule
$t_{\text{latent}}$ & \# latents & \# images \\ \midrule
\num{3e-3}   & \num{9418}       & \num{485}     \\
\num{6e-3} & \num{895} & \num{359} \\
\num{1e-2}   & \num{20}         & \num{23}      \\ \bottomrule
\end{tabular}
\label{tab:data_gen_trait_thresh}
\end{table}


==> tables/qwen7_72_tbl.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{
    We investigate the effect of the verbalizer MLLM for morphological trait extraction for both the MLLM-only and MLLM + SAE models.
    The larger Qwen-2.5-VL-72B model \cite{Qwen2VL} consistently obtains better ratings than its 7B counterpart.
    We note that Qwen-2.5-VL-7B might lead to false positives due to hallucination while extracting common traits in three input SAE-annotated images (Figure~\ref{fig:qwen7_vs_qwen72}).
    In contrast, the Qwen2.5-VL-72B model demonstrates improved robustness, avoiding such hallucinations and yielding more accurate trait descriptions.
    The experimental setup uses an input dataset of 20K images and $t_{\text{freq}}$ = \num{1e-2}. 
    }\label{tab:mllm-quality}
    \begin{tabular}{lrrrr}
        \toprule
        \bfseries Method & \bfseries MLLM & \bfseries \# Images & \bfseries \# Traits & \bfseries Avg.\ Rating \\
        \midrule
        MLLM & Qwen-2.5 VL 7B & \num{476} & \num{536} & \num{2.85} \\
        MLLM & Qwen-2.5 VL 72B & \num{371} & \num{411} & \num{3.15} \\
        \midrule
        MLLM + SAE & Qwen-2.5 VL 7B & \num{478} & \num{538} & \num{2.90} \\
        MLLM + SAE & Qwen-2.5 VL 72B & \num{358} & \num{370} & \textbf{\num{3.58}} \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/stats_hyperparam.tex <==
\noindent
\begin{minipage}{0.38\linewidth}
\centering
% \begin{table}[htbp]
% \centering
\small
\captionof{table}{Dataset statistics. On average, each image is associated with $4.2$ trait samples.}
\label{tab:data_stat}
\begin{tabular}{@{}ll@{}}
\toprule
\bfseries Metric                & \bfseries Value \\ \midrule
\# Species         & \num{736}   \\
\# Genera          & \num{417}   \\
\# Unique   images & \num{19.1}K \\ \midrule
\# Samples         & \num{80.8}K \\
\bottomrule
\end{tabular}
% \end{table}
\end{minipage}
\hfill
\begin{minipage}{0.6\linewidth}
\centering
% \begin{table}[htbp]
    % \centering
    \small
    \captionof{table}{Hyperparameters for SAE training and filtering.}
    \begin{tabular}{lr}
        \toprule
        \bfseries Hyperparameter & \bfseries Value \\ 
        \midrule
        Hidden Width & \num{24576} ($32\times$ expansion) \\
        Sparsity Coefficient $\alpha$ & \num{2e-4}, \num{4e-4}, \num{8e-4} \\
        Sparsity Coefficient Warmup & \num{500} steps \\
        Batch Size & \num{16384} \\
        Learning Rate $\eta$ & \{\num{5e-4}, \num{1e-3}\} \\
        Learning Rate Warmup & \num{500} steps \\
        Activation threshold $t_{\text{activation}}$ & 0.9 \\
        \bottomrule
    \end{tabular}
    \label{tab:hyperparam}
% \end{table}
\end{minipage}
